Semantic Pyramid for Image Generation

We present a novel GAN-based model that utilizes the space of deep features learned by a pre-trained classification model. Inspired by classical image pyramid representations, we construct our model as a Semantic Generation Pyramid -- a hierarchical framework which leverages the continuum of semantic information encapsulated in such deep features; this ranges from low level information contained in fine features to high level, semantic information contained in deeper features. More specifically, given a set of features extracted from a reference image, our model generates diverse image samples, each with matching features at each semantic level of the classification model. We demonstrate that our model results in a versatile and flexible framework that can be used in various classic and novel image generation tasks. These include: generating images with a controllable extent of semantic similarity to a reference image, and different manipulation tasks such as semantically-controlled inpainting and compositing; all achieved with the same model, with no further training.

==> abstract.tex <==
\begin{abstract}
We propose a novel image generation model that works in full conjunction with features extracted from a pre-trained classification network. Our model is designed and trained to utilize the hierarchical representation and semantic information encoded in such features via a unified Generative Adversarial Network (GAN) based framework. Given a set of features extracted from an input image, our model can generate diverse image samples, each with matching features at each semantic level of the classification model.  This is in contrast to existing optimization-based methods that are able to reconstruct only a single average image and are often limited in the type of features they can invert. \tali{this following sentence repeats a bit what we said before..} Our unified framework goes beyond that and allows to explore the distribution of images matching to features from different semantic levels. We further demonstrate the versatility and applicability of our model through a number of tasks including  image generation with a controllable extent of semantic similarity to a given image, and various semantically-aware image manipulation tasks -- all achieved with the same model, with no additional information or further training.

\end{abstract}
  %Deep features, extracted from hidden layers of Convolutional Neural Networks (CNNs) were shown to encode meaningful information. This observation gave rise to various manipulations on these features. Inverting features back to pixels is crucial in order to project the semantic manipulations to new output images. This procedure has mostly been done by an iterative optimization process which is very limited; Since it assumes one correct reconstruction exists, it convergence to an implausible expectation. This has been addressed so far mostly by imposing regularization priors on the reconstructed image, which often leads to blurry unrealistic reconstructions and limits the type of features that can be used. In this work, we propose inverting deep features by a Generative Adversarial Network (GAN). We do so by using a generator that is a mirror of the recognition model and trains adversarialy to produce various results matching to each semantic level of the recognition model. This approach gives rise to image representation as a Semnatic-Pyramid and obtain the change in the distribution of images when manipulating different levels of the pyramid. \todo{I would like to express something about having both better interpretability (understanding featuremap-condtioned distribution due to diversity) and better manipulation and inverting}https://www.overleaf.com/8774791258rkxyxszjrgcj

==> introduction_backup.tex <==
\section{Introduction}
%motivation
Convolutional Neural Networks (CNNs) trained for classification have come a long way in recent years, and are now capable of achieving impressive classification results for a variety of real-world objects in natural environments.  Furthermore, it has been shown that such classification models learn powerful and meaningful feature spaces, encoding not only objects' class, but also rich information ranging from low level features  to high-level semantic content~\cite{alexnet}. Such features have been widely utilized by numerous methods for clustering, perceptual loss \cite{zhang2018perceptual} and different image manipulation tasks (e.g., \cite{Upchurch_2017, style_transfer, Johnson_2016, arar2019image}). 

 % previous work
The process of working in feature space typically involves the following stages: an image is fed to a pre-trained classification network (e.g., VGG-19); its feature responses from different layers are extracted, and  manipulated according to the application in hand. The manipulated features are then inverted back to  an image  by solving a reconstruction optimization problem. However, the problem of inverting deep features into a realistic image is challenging -- there is no one-to-one mapping between the deep features and an image, especially when the features are taken from deep layers. This has been addressed so far mostly by imposing regularization priors on the reconstructed image, which often leads to blurry unrealistic reconstructions and limits the type of features that can be used. 

% ours: utilize the VGG feature space in generative model.
In this paper, we take a different route -- we propose a novel image generative model that intertwine features learned by a pre-trained classification model with recent advances in generative adversarial networks (GANs).  Our model effectively leverages the hierarchical representation learned by classification models, yet avoids imposing any image priors, but rather learns such priors from the data using adversarial training. More specifically, given a set of input features from different levels, our model  generates a \emph{diverse} set of realistic image samples that match the input features. This is in contrast to existing optimization-based methods that reconstruct only a single average image. % Furthermore, such methods do not model 

\tali{Talk about differences from existing GANs methods. Exisiting GANs }
Our model maps a 1D random vector into a realistic image sample. However, differently from traditional GANs, it works in  full conjunction with the pre-trained classification model -- its architecture is a mirror of the classification model, where at each level it can receive as input the corresponding feature map. The model learns to fuse the input features and to invert them into realistic image samples. Due to the hierarchical nature of the input features, this results in a \emph{Semantic Pyramid Generation} model which has several key properties: (i) \emph{semantic controllability} --  given a source image, we can generate additional image samples with a gradual, controllable semantic similarity to the source (see Fig.~\ref{fig:teaser}). (ii)  Motivated by classical image pyramid representations (e.g., Laplacian pyramids), we demonstrate the  use of our model in a variety of \emph{semantically-aware image manipulation tasks}, including semantically-controlled inpainting, semantic harmonization of objects into images, and diverse image-to-image translation like colorization of grayscale images, generating realistic images from line-drawings and more. For all these tasks, we can control and edit features at different semantic levels and still produce realistic image samples from the manipulated features. 
All our generation results are achieved with the same model without any further optimization or fine tuning. 


\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{figures/inversion4.pdf}
    \caption{{\bf Random image samples from increasing semantic levels.} For each input image (top row), we show random image samples generated by our model when fed with deep features from increasing semantic levels (top to bottom). Our model generates realistic image samples, where the similarity to the original image is controlled by the level of the input features --- the deeper the features' level is, the more we can deviate from the original image. For all generation levels, our model preserves the semantic content of the input image and produces high quality diverse image samples.}
    \label{fig:inversion}
\end{figure*}




% (1)  continuum leverage features from different levels 
% (2)   avoid optimization, leverage GANs




% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\textwidth]{figures/image_manipulation.pdf}
%     \caption{{\bf Semantic pyramid image manipulation.} }
%     \label{fig:im_manipulation}
% \end{figure*}



% \begin{itemize}
%     \item Classification using CNN achieves great results (cite some). The feature-maps are meaningful (cite clustering and nearest neighbor stuff).
%     \item The fact that they are meaningful motivated many researchers to make use both for interpretability: 
%     Vedaldy inverting \cite{Mahendran_2015}, 
%     BroxGAN \cite{Dosovitskiy:2016:GIP:3157096.3157170}, 
%     BroxConvs \cite{DBLP:journals/corr/DosovitskiyB15}, 
%     Net dissection \cite{netdissect2017}.
%     and for image manipulation:
%     Noah \cite{Upchurch_2017},
%     Gatys \cite{style_transfer},
%     Johnson style \cite{Johnson_2016},
%     deep seam carving \cite{arar2019image},
%     \item We are inspired by classical image manipulation using laplacian pyramids. 
%     \cite{Burt83thelaplacian},
%     \cite{adelson1984pmi}.
%     but want to use the semantic analogy to those, to allow semantic manipulation.
%     \item For that sake we are interested in inverting deep features back to images in the pixel-space.
%     \item As oppose to previous approaches for inverting which are discriminative (i.e. tryin to find the closest image to the unknown input by expectation), we employ a generative model, understanding that mapping to deep features is a many-to-one problem and therefore inverting means estimating a distribution of possible solutions and sampling out of it.
%     \item To achieve that we use GAN \cite{GAN}. GANs achieved great results during the last years \cite{dcgan}, \cite{SAGAN}, \cite{BIGGAN}, \cite{progan}, \cite{stylegan}. Also for image to image tasks: \cite{pix2pix2017}, \cite{pix2pixHD}, \cite{cyclegan}, \cite{munit}.
%     \item While attempts of manipulating and interpreting GANs were made \cite{bau2019gandissect}, \cite{isola-latentspace}, We explore the relation between generative models and semantic discriminative models. We invert a classifier using a GAN.
%     \item This allows generation by reference: Given an image we generate another one which is semnatically-similar to the input to a controllable extent (see figs).
%     \item Moreover, inspired by lap-pyramids, we demonstrate various semantic manipulations on images, by expressing the as a pyrmaid of semantic content descriptions.
%     \item We evaluate our results by incscore, FID and MOS.
%     \item Specify contributions?
% \end{itemize}
